Science cases for a visible interferometer

High spatial resolution is the key for the understanding various astrophysical phenomena. But even with the future E-ELT, single dish instruments are limited to a spatial resolution of about 4 mas in the visible. For the closest objects within our Galaxy most of the stellar photosphere remains smaller than 1 mas. With the success of long baseline interferometry these limitations were soom overcome. Today low and high resolution interferometric instruments on the VLTI and CHARA offer an immense range of astrophysical studies. Combining more telescopes and moving to visible wavelengths broadens the science cases even more. With the idea of developing strong science cases for a future visible interferometer, we organized a science group around the following topics: pre-main sequence and main sequence stars, fundamental parameters, asteroseismology and classical pulsating stars, evolved stars, massive stars, active galactic nuclei (AGNs) and imaging techniques. A meeting was organized on the 15th and 16th of January, 2015 in Nice with the support of the Action Specific in Haute Resolution Angulaire (ASHRA), the Programme National en Physique Stellaire (PNPS), the Lagrange Laboratory and the Observatoire de la Cote d'Azur, in order to present these cases and to discuss them further for future visible interferometers. This White Paper presents the outcome of the exchanges. This book is dedicated to the memory of our colleague Olivier Chesneau who passed away at the age of 41.

==> EVOL_nardetto/friend_pulsantes_nn_v0.tex <==
\chapter[Visible interferometry of $\delta$ Scuti and RR Lyrae stars]{Visible interferometry of $\delta$ Scuti and RR Lyrae stars}}

%\documentclass{aa}  
%\usepackage{graphicx}
%\usepackage{natbib}
%\usepackage{hyperref}
%\usepackage{color}

%\titlerunning{}

\def\te{T_{\rm eff}}
\def\Mo{M_{\odot}}
\def\Lo{L_{\odot}}
\def\Ro{R_{\odot}}
\def\deg{\ensuremath{^\circ}}
\newcommand{\ep}[1]{\textcolor{red}{#1}}
\newcommand{\astroph}[1]{astro-ph/{#1}}
\newcommand{\AJ}[3]{{#1}, AJ, \vol{{#2}}, {#3}}
\newcommand{\ApJ}[3]{{#1}, ApJ, \vol{{#2}}, {#3}}
\newcommand{\ApJS}[3]{{#1}, ApJS, \vol{{#2}}, {#3}}
\newcommand{\ApJLett}[3]{{#1}, ApJ, \vol{{#2}}, {#3}}
\newcommand{\ApJL}[3]{{#1}, ApJ, \vol{{#2}}, {#3}}
\newcommand{\AnnRev}[3]{{#1}, Annual Review of Astron. and Astrophys.,
\vol{{#2}}, {#3}}
\newcommand{\AandA}[3]{{#1}, A\&A, \vol{{#2}}, {#3}}
\newcommand{\AandAsupp}[3]{{#1}, A\&A Supp.\rm, \vol{{#2}}, {#3}}
\newcommand{\AN}[3]{{#1}, Astron. Nachr.\rm, \vol{{#2}}, {#3}}
\newcommand{\MNRAS}[3]{{#1}, MNRAS\rm, \vol{{#2}}, {#3}}
\newcommand{\MmSAI}[3]{{#1}, Mem. Soc. Astron. Ital.\rm, \vol{{#2}},
{#3}}
\newcommand{\Mess}[3]{{#1}, The Messenger\rm, \vol{{#2}}, {#3}}
\newcommand{\Vistas}[3]{{#1}, Vistas Astr.\rm, \vol{{#2}}, {#3}}
\newcommand{\Observatory}[3]{{#1}, Observatory\rm, \vol{{#2}}, {#3}}
\newcommand{\PASP}[3]{{#1}, PASP\rm, \vol{{#2}}, {#3}}
\newcommand{\PASPC}[3]{{#1}, PASPC\rm, \vol{{#2}}, {#3}}
\newcommand{\PASJ}[3]{{#1}, PASJ\rm, \vol{{#2}}, {#3}}
\newcommand{\vol}[1]{{\mbox{#1}}}

\newcommand{\Teff}{\mbox{$T_{\mbox{\scriptsize eff}}\,$}}
\newcommand{\Tefffour}{\mbox{$T^{4}_{\mbox{\scriptsize eff}}\,$}}
\newcommand{\Teq}{\mbox{$T_{\mbox{\scriptsize eq}}\,$}}
\newcommand{\Sv}{\mbox{$S_{V}\,$}}
\newcommand{\BCv}{\mbox{$\mbox{B.C.}_{V}\,$}}
\newcommand{\geff}{\mbox{$g_{\mbox{\scriptsize eff}}\,$}}
\newcommand{\Vrot}{\mbox{$v_{\mbox{\scriptsize rot}}\,$}}
\newcommand{\mbol}{\mbox{$m_{\mbox{\scriptsize bol}}\,$}}
\newcommand{\mv}{\mbox{$m_{V}\,$}}
\newcommand{\mk}{\mbox{$m_{K}\,$}}
\newcommand{\Mbol}{\mbox{$M_{\mbox{\scriptsize bol}}\,$}}
\newcommand{\Mb}{\mbox{$M_{B}\,$}}
\newcommand{\Mv}{\mbox{$M_{V}\,$}}
\newcommand{\Mk}{\mbox{$M_{K}\,$}}
\newcommand{\Mh}{\mbox{$M_{H}\,$}}
\newcommand{\Mj}{\mbox{$M_{J}\,$}}
\newcommand{\Mi}{\mbox{$M_{I}\,$}}
\newcommand{\Mw}{\mbox{$M_{W}\,$}}
\newcommand{\Wvi}{\mbox{$W_{VI}\,$}}
\newcommand{\Wjk}{\mbox{$W_{JK}\,$}}
\newcommand{\Mrr}{\mbox{$M_{\mbox{\scriptsize RR}}\,$}}
\newcommand{\delMv}{\mbox{$\Delta
         M_{\mbox{\scriptsize V,TO}}^{\mbox{\scriptsize RR}}\,$}}
\newcommand{\meanMbol}{\mbox{$<\!\!M_{\mbox{\scriptsize bol}}\!\!>\,$}}
\newcommand{\meanMv}{\mbox{$<\!\!M_{V}\!\!>\,$}}
\newcommand{\meanMk}{\mbox{$<\!\!M_{K}\!\!>\,$}}
\newcommand{\Koff}{\mbox{$K_{\mbox{\scriptsize off}}\,$}}
\newcommand{\MvRR}{\mbox{$<M_{V}(RR)>\,$}}
\newcommand{\MkRR}{\mbox{$<M_{K}(RR)>\,$}}
\newcommand{\MbolRR}{\mbox{$<M_{\mbox{\scriptsize bol}}(RR)>\,$}}
\newcommand{\MvTO}{\mbox{$M_{V}(TO)\,$}}
\newcommand{\RRab}{\mbox{$RR{\mbox{\scriptsize ab}}\,$}}
\newcommand{\RRc}{\mbox{$RR{\mbox{\scriptsize c}}\,$}}
\newcommand{\RRd}{\mbox{$RR{\mbox{\scriptsize d}}\,$}}
\newcommand{\pmag}{\mbox{$\stackrel{\mbox{\scriptsize m}}{\textstyle
.}$}}
\newcommand{\mags}{\mbox{$^{\mbox{\scriptsize m}}$}}
\newcommand{\pday}{\mbox{$\stackrel{\mbox{d}}{\textstyle .}$}}
\newcommand{\pperiod}{\mbox{$\stackrel{p}{\textstyle .}$}}
\newcommand{\phour}{\mbox{$\stackrel{h}{\textstyle .}$}}
\newcommand{\hours}{\mbox{$^{h}$}}
\newcommand{\pmin}{\mbox{$\stackrel{m}{\textstyle .}$}}
\newcommand{\mins}{\mbox{$^{m}$}}
\newcommand{\psec}{\mbox{$\stackrel{s}{\textstyle .}$}}
\newcommand{\secs}{\mbox{$^{s}$}}
\newcommand{\parcsec}{\mbox{$\stackrel{\prime\prime}{\textstyle .}$}}
\newcommand{\arcsecs}{\mbox{$^{\prime\prime}$}}
\newcommand{\parcmin}{\mbox{$\stackrel{\prime}{\textstyle .}$}}
\newcommand{\arcmins}{\mbox{$^{\prime}$}}
\newcommand{\solar}{\mbox{$\odot$}}
\newcommand{\Rsolar}{\mbox{$R_{\odot}\,$}}
\newcommand{\Msolar}{\mbox{$\vec{M}_{\odot}\,$}}
\newcommand{\Lsolar}{\mbox{$L_{\odot}\,$}}
\newcommand{\Tsolar}{\mbox{$T_{\odot}\,$}}
\newcommand{\FeH}{\mbox{[Fe/H]}\,}
\newcommand{\OFe}{\mbox{[O/Fe]}\,}
\newcommand{\kms}{\mbox{$\mbox{km\,s}^{-1}$}\,}
\newcommand{\Mpc}{\mbox{Mpc}\,}
\newcommand{\prMpc}{\mbox{$\mbox{Mpc}^{-1}$}\,}
\newcommand{\logg}{\mbox{$\log (g)$}\ }
\newcommand{\loggzero}{\mbox{$\log (g_0)$}\ }
\newcommand{\logP}{\mbox{$\log P$}\ }
\newcommand{\mM}{\mbox{$(m-M)$}\ }
\newcommand{\mMzero}{\mbox{$(m-M)_0$}\ }
\newcommand{\thetaspec}{\mbox{$\theta_{\mbox{\scriptsize spec}}$}}
\newcommand{\thetaphot}{\mbox{$\theta_{\mbox{\scriptsize phot}}$}}
\newcommand{\Smin}{\mbox{$\Sigma_{\mbox{\scriptsize min}}$}\,}
\newcommand{\Ab}{\mbox{$\mbox{A}_{\mbox{\scriptsize B}}$}\,}
\newcommand{\vrad}{\mbox{$\mbox{v}_{\mbox{\scriptsize rad}}$}\,}
\newcommand{\hubble}{\mbox{$H_{\mbox{\scriptsize 0}}\:$}}
\newcommand{\phase}[2]{\mbox{[{#1};{#2}]}\,}
\newcommand{\magdex}{\mbox{mag~dex$^{-1}$}\,}
\newcommand{\thetaLD}{\mbox{ $\theta_{\mbox{\scriptsize LD}}$}\,}
\newcommand{\Fv}{\mbox{ $F_{\mbox{\scriptsize V}}$}\,}

\begin{document}

\title{Prospective about the visible interferometry \\ of $\delta$ Scuti and RR Lyrae stars}

\titlerunning{Prospective about the visible interferometry of pulsating stars (except Cepheids)}
\authorrunning{Nardetto et al. }

\author{N. Nardetto \inst{1}}

\institute{Laboratoire Lagrange, UMR7293, Universit\'e de Nice Sophia-Antipolis, CNRS, Observatoire de la C\^ote d'Azur, Nice, France Nicolas.Nardetto@oca.eu   \and  
}

\date{Received ... ; accepted ...}

\abstract{The Baade-Wesselink method of distance determination is usually applied to Cepheids because they are bright. But with a new generation of very sensitive long-baseline visible interferometers (in north and south hemispheres), and with also the upcoming of Gaia, it seems now of great interest to study fainter pulsating stars like RR Lyrae or $\delta$~Scuti stars, which also stand into the instability strip. In particular, the projection factor which is used in the BW method is totally understood for these kind of stars.} 
{Using Gaia parallaxes, we propose to derive the period-projection factor relation of RR Lyrae and $\delta$-Scuti stars, by applying the inverse BW method. } 
{In the BW method, the projection factor is usually assumed while the distance is derived. But if we know the distance, we can infer the projection factor. For this, we need an independent measurement of the angular diameter curve, which can be provided by future visible interferometer. }
{The knowledge of the projection factor of $\delta$-Scuti stars and RR Lyrae will provide crucial informations about their physical structure: limb-darkening variation, atmospheric velocity gradient, dynamical structure of their atmosphere. And a comparison with Cepheids is interesting to better understand their physical nature, and ultimately better control the systematics in the BW method.} 
{Once the \emph{Pp} relations calibrated, one can apply more easily the photometric version of the BW method for many fainter objects, which helps also (together with Gaia) to constrain the \emph{PL} relation for these objects which is of very hight interest for several reasons, and one of them is the study of global clusters. }

\keywords{Techniques: interferometry -- Stars: circumstellar matter -- Stars:
oscillations (including pulsations) }

%\maketitle

\section{The projection factor of $\delta$ Scuti and RR Lyrae stars}

The Baade-Wesselink (BW) method has been widely used to calibrate the period-luminosity relation of Cepheids \citep{fouque07, storm11a, storm11b} with important implications for the extragalactic distance scale and
cosmology \citep{riess11}. It has been applied for Cepheids using interferometry \citep{kervella04a, davis09} and photometry \citep{gieren05}, but also for RR Lyrae stars \citep{fernley94} and $\delta$~Scuti stars \citep{wilson93, milone94,  wilson98}. Concerning $\delta$ Scuti stars a radial pulsation is required to apply the {\it classical} BW method. Many High-Amplitude $\delta$-Scuti (hereafter HADS) stars show radial fundamental mode of pulsation (combined sometimes with other harmonics). These are the best candidates to apply the BW analysis. However, few studies have been done in this field and the parallaxes of Hipparcos currently remains the only geometric method that has been used to calibrate their \emph{PL} relations \citep{petersen98}.

The basic principle of the BW method is to compare the linear and
angular size {\it variation} of a pulsating star in order to derive
its distance through a simple division. The key point is that
photometric measurements lead to angular diameters corresponding to the {\it
photospheric} layer, while the linear stellar radius variation is
deduced by spectroscopy, i.e., based on line-forming regions which
form higher in the atmosphere. Thus, radial velocities
$V_{\mathrm{rad}}$, which are derived from line profiles, include
the integration in two directions: over the stellar surface through
limb-darkening and over the atmospheric layers through velocity
gradients. All these phenomena are currently merged in one specific
quantity, generally considered constant with time: the projection
factor $p$, defined as $V_{\mathrm{puls}}=pV_{\mathrm{rad}}$, where
$V_{\mathrm{puls}}$ is defined as the {\it photospheric} pulsation
velocity \citep{nardetto04}. $V_{\mathrm{puls}}$ is then
integrated with time to derive the photospheric radius
variation.

\begin{figure}[htbp]
\begin{center}
\resizebox{1.0\hsize}{!}{\includegraphics[clip=true]{fig1_Pp.eps}}
\end{center}
\caption{The Baade-Wesselink projection factor as a function of the period for different kinds of pulsating stars. The $\delta$~Scuti stars indicated as blue diamonds are, by increasing period: $\beta$~Cas, DX~Cet, AI~Vel and $\rho$~Pup.} \label{Fig2}
\end{figure}

The projection factor appears widely in the literature for Cepheids. Up to recently, a
constant geometric projection factor was commonly used for all kinds
of pulsating stars (generally $p=1.36$, \citet{burki82}). Using high
precision spectroscopic measurements of 10 southern hemisphere Galactic
Cepheids with HARPS, we measure directly the velocity gradient
within the atmosphere of Cepheids and derive semi-theoretical
$p$-factors. We discovered a relation between the period of Cepheids
and the projection factor. We also showed that if one uses a
constant $p$-factor ($p=1.36$) to derive the \emph{PL} relation,
errors of $0.10$ and $0.03$ on the slope and zero-point of the
\emph{PL} relation can be introduced. This means that distances can
be overestimated by 10\% for long-period Cepheids \citep{nardetto07, nardetto09}.


The aim of this proposal is to derive the expected period-projection factor relation of RR Lyrae and High-Amplitude $\delta$ Scuti stars (HADS) by applying the inverse BW method. HADS are generally supposed to pulsate radially. However, weak non-radial pulsation could be detected using long baseline visible interferometry. 
In that case, the Baade-Wesselink method, if revised, can constitute an interesting tool to distinguish radial and non-radial modes of pulsation. \citet{balona79a, balona79b, balona79c} and \citet{stamford81} give a $p$-factor estimates connected to the non-radial mode of the star, while the classical approach done for Cepheids have been recently applied to several $\delta$-Scuti with dominant radial mode \citet{guiglion13, nardetto14}.


\begin{figure}[htbp]
\begin{center}
\resizebox{1.0\hsize}{!}{\includegraphics[clip=true]{fig2_PL.pdf}}
\end{center}
\caption{ Period-Luminosity relation of Galactic $\delta$~Scuti (lower magnitude) and Cepheid (larger magnitude) variable stars (figure from Mc Namara et al. 2007).  The PL relation of Cepheids combined with the PL relation of $\delta$~Scuti stars would provide an interesting tool for the extragalactic distance scale.} \label{Fig2}
\end{figure}

Once the projection factor derived, the photometric version of the BW method can be applied to a wider sample of fainter $\delta$~Scuti and RR Lyrae stars, and, with the combination of Gaia parallaxes, this can help to provide a robust period-luminosity relation. Deriving such relation is extremely interesting for different reasons. First, \citep{fernie92} and then \citep{mcnamara07} showed that the PL relation of $\delta$~Scuti stars and Cepheids seems to be consistent in slope and zero-point ({\ref{Fig2}). Second, Cepheids are
supergiant stars and are relatively rare in space, while $\delta$-Scuti stars are dwarf or near-dwarf stars and are numerous in the solar neighborhood. Many are so nearby that they have negligible or very small reddening. Third, SX Ph stars can be found in Globular Clusters, that helps also to constrain the PL relation of RR Lyrae  \citep{mcnamara07}. The PL relation of Cepheids combined with the PL relation of $\delta$~Scuti stars would provide an interesting tool to the extragalactic distance scale. And if we show that the BW method can be used to calibrate the PL relation of $\delta$~Scuti using a specific p-factor (and in a consistent way compared to trigonometric measurements) it will open a new and promising field of investigation. 

\begin{table}[htbp] \caption{\label{Tab.ang} HADS and RR Lyrae}
\begin{center}
\begin{tabular}{lccc|ccccccccc}
\hline
\hline
N$_\star$	& $\simeq$ 10 \\
spatial resolution 	& $\theta$ from 0.1 to 0.25 mas \\
spectral resolution 	&  $R=3000$ \\			
temporal resolution	&  10 minutes (high sensitivity required) \\
precision 	&	1\% at low visibilities \\	
imaging	& 3T is fine, 6T is best \\
\hline
\end{tabular}
\end{center}
%\begin{list}{}{}
%\item[$^{\mathrm{a}}$]  and/or minimum number of telescopes required
%\end{list}
\end{table}

\section{Pulsating stars in binaries}

Another very interesting aspect is to study pulsating stars in binaries in order to (1) measure their orbital solution with interferometry and (2) derive their mass, which put important constrains on the evolutionary models. it concerns not only  $\delta$ Scuti stars, but also RR Lyrae, $\beta$ Cepheids, $\gamma$ Dor and RoAp stars.  From Garcia et al. (1995), Stankov et al. (2005) and Matthews et al. (1999), together with the Galactic Variable Catalogue, we found about 140 objects to be observed with $mV <7$ and 200 objects with $mV <9$. The exact orbital separation still have to be calculated to better characterize how many objects could be resolved by a 300 meters baseline interferometer.

 
\bibliographystyle{aa}  % A&A bibliography style file (aa.bst)
\bibliography{bibtex} % your references in file: Yourfile.bib
 


\end{document}


==> bibliography.tex <==
\begin{thebibliography}{99}

\bibitem[{\AmS(2004)}]{ams04}
\AmS (2004). \emph{\AmS-\LaTeX{} Version 2 User's Guide} (American Mathematical
  Society, Providence), \url{http://www.ams.org/tex/amslatex.html}.

\bibitem[{Baker and Carter(1972)}]{bake72}
Baker, D.~W. and Carter, N.~L. (1972). \emph{Seismic Velocity Anisotropy
  Calculated for Ultramafic Minerals and Aggregates}, \emph{Geophys.
  Mono.}, Vol.~16 (Am. Geophys. Union), pp. 157--166.

\bibitem[{Benhamou and Colmerauer(1993)}]{benh93}
Benhamou, F. and Colmerauer, A. (eds.) (1993). \emph{Constraint Logic
  Programming, Selected Research} (MIT Press).

\bibitem[{Bestbury(2003)}]{best03}
Bestbury, B.~W. (2003). {$R$}-matrices and the magic square, \emph{J.
  Phys. A} \textbf{36}, 7, pp. 1947--1959.

\bibitem[{Brown(1988)}]{brow88}
Brown, M.~E. (1988). \emph{An interactive environment for literate
  programming}, Ph.D. thesis, Texas A\&M University, TX, USA.

\bibitem[{Churchill and Brown(1990)}]{chur90}
Churchill, R.~V. and Brown, J.~W. (1990). \emph{Complex {V}ariables and
  {A}pplications}, 5th edn. (McGraw-Hill).

\bibitem[{Davidsen(1993)}]{davi93}
Davidsen, B. (1993). Netpbm,
  \url{ftp://ftp.wustl.edu/graphics/graphics/packages/NetPBM}.

\bibitem[{Deligne and Gross(2002)}]{pier02}
Deligne, P.~X. and Gross, B.~H. (2002). On the exceptional series, and
  its descendants, \emph{C. R. Math. Acad. Sci. Paris} \textbf{335}, 11, pp.
  877--881.

\bibitem[{Gupta and Senturia(1997)}]{gupt97}
Gupta, R.~K. and Senturia, S.~D. (1997). Pull-in time dynamics as a
  measure of absolute pressure, in \emph{Proc. IEEE Int. Workshop
  on Microelectromechanical Systems (MEMS'97)} (Nagoya, Japan), pp. 290--294.

\bibitem[{Heard \emph{et~al.}(1994)Heard, Borg, Carter and Raleigh}]{hear94}
Heard, H.~C., Borg, I.~V., Carter, N.~L. and Raleigh, C.~B. (1994).
  {VoQS: Voice Quality Symbols}, Revised to 1994.

\bibitem[{Hobby(1992)}]{hobb92}
Hobby, J.~D. (1992). {A User's Manual for MetaPost}, Tech. Rep. 162,
  AT\&T Bell Laboratories, Murray Hill, New Jersey.

\bibitem[{Jarlskog(1988)}]{jarl88}
Jarlskog, C. (1988). \emph{CP {V}iolation} (World Scientific, Singapore).

\bibitem[{Jones(1973)}]{dani73}
Jones, D. (1973). {The term `phoneme'}, in W.~E. Jones and J.~Laver
  (eds.), \emph{Phonetics in Linguistics: A Book of Reading} (Longman, London),
  pp. 187--204.

\bibitem[{Kernighan(1984)}]{bria84}
Kernighan, B.~W. (1984). {PIC}---{A} graphics language for
  typesetting, Computing Science Technical Report 116, AT\&T Bell
  Laboratories, Murray Hill, New Jersey.

\bibitem[{Lamport(1987)}]{lamp87}
Lamport, L. (1987). \emph{Make Index: An Index Processor For LaTeX}.

\bibitem[{Lamport(1994)}]{lamp94}
Lamport, L. (1994). \emph{\LaTeX, A Document Preparation System}, 2nd edn.
  (Addison-Wesley, Reading, MA).

\bibitem[{Landsberg and Manivel(2002)}]{jame02}
Landsberg, J.~M. and Manivel, L. (2002). Triality, exceptional {L}ie
  algebras and {D}eligne dimension formulas, \emph{Adv. Math.} \textbf{171},
  1, pp. 59--85, \url{http://www.url.com/triality.html}.

\bibitem[{Lodha(1974)}]{lodh74}
Lodha, G.~S. (1974). \emph{Quantitative interpretation of ariborne
  electromagnetic response for a spherical model}, Master's thesis, University
  of Toronto, Canada.

\bibitem[{Richardson(1960)}]{rich60}
Richardson, L.~F. (1960). \emph{Arms and {I}nsecurity} (Boxwood, Pittsburg).

\bibitem[{Weiss(1994)}]{weis94}
Weiss, G.~H. (ed.) (1994). \emph{Contemporary {P}roblems in {S}tatistical
  {P}hysics} (SIAM, Philadelphia).

\end{thebibliography}


==> chapter2.tex <==
\chapter[\btex ing Using the WSPC {\bib}Style]{\btex ing\\[.5ex] Using the \\[.5ex] WSPC {\bib}Style\label{ch2}}

\section{\btex{} Database Entries}

\begin{center}
\tablefont
\begin{tabular}{@{}ll@{}}\toprule
\multicolumn{1}{c}{\btex}\\
\multicolumn{1}{c}{Database}  & \multicolumn{1}{c}{Sample citation}\\
\multicolumn{1}{c}{entry type}\\\colrule

article & \cite{best03,pier02}\\

proceedings & \cite{weis94}\\

inproceedings & \cite{gupt97}\\

book & \cite{rich60,jarl88}\\

edition & \cite{chur90}\\

editor & \cite{benh93}\\

series & \cite{bake72}\\

tech report & \cite{hobb92}\\

unpublished & \cite{hear94}\\

phd thesis & \cite{brow88}\\

masters thesis & \cite{lodh74}\\

incollection & \cite{dani73}\\

misc & \citep[Theorem 2.1]{davi93}\\
\botrule
\end{tabular}
\end{center}

\section{\btex}\index{\btex}
If you use the \btex\ program to maintain your bibliography, you do
not use the \verb|thebibliography| environment. Instead, you should
include the lines

\begin{verbatim}
   \bibliographystyle{ws-book-har}
   \bibliography{ws-book-sample}
\end{verbatim}

\noindent where \verb|ws-book-har| refers to a file
\verb|ws-book-har.bst|, which defines how your references will look.

The argument to \verb|\bibliography| refers to the file \verb|ws-book-sample.bib|,
which should contain your database in \btex\ format. Only the
entries referred to via \verb|\cite| will be listed in the
bibliography.

\newpage

To complete the job, compile your file as follows:

\begin{enumerate}[(6)]
\item \verb|latex ws-book975x65|
\item \verb|latex ws-book975x65|
\item \verb|bibtex ws-book975x65|
\item \verb|makeindex ws-book975x65|
\item \verb|latex ws-book975x65|
\item \verb|latex ws-book975x65|
\end{enumerate}


==> chapter3.tex <==
\chapter{Indexing\label{ch3}}

\section{Indexing}\index{index}
The first step in producing the index is to put the necessary
\verb|\index| commands in your document. The following example shows
some simple \verb|\index| commands and the index entries that they
produce.

\begin{table}[h]
\begin{tabular}{ll|l}
Page ii:   & \verb|\index{Alpha}              | &  Alpha, ii           \\
Page viii: & \verb|\index{alpha}              | &  alpha, viii, ix, 22 \\
Page ix:   & \verb|\index{alpha}              | &  bites               \\
Page 7:    & \verb|\index{gnat!size of}       | &  \sitem animal       \\
Page 8:    & \verb|\index{bites!animal!gnats} | &  \ssitem gnats, 8, 10\\
Page 10:   & \verb|\index{bites!animal!gnats} | &  \ssitem gnus, 10    \\
Page 10:   & \verb|\index{bites!animal!gnus}  | &  \sitem vegetable, 12\\
Page 12:   & \verb|\index{bites!vegetable}    | &  gnat, 32            \\
Page 22:   & \verb|\index{alpha}              | &  \sitem anatomy, 35  \\
Page 32:   & \verb|\index{gnat}               | &  \sitem size of, 7   \\
Page 35:   & \verb|\index{gnat!anatomy}       | &  gnus                \\
           & \verb|\index{gnus!good}          | &  \sitem bad, 38      \\
Page 38:   & \verb|\index{gnus!bad}           | &  \sitem good, 35
\end{tabular}
\end{table}

You then run \LaTeX\ on your entire document, causing it to generate
the file {\tt ws-book975x65.idx}. Next, run the \verb|MakeIndex|
program by typing the command, \verb|makeindex ws-book975x65|. This
produces the file \verb|ws-book975x65.ind|. If \verb|MakeIndex|
generated no error messages, you can now rerun \LaTeX\ on your
document and the index will appear.

Reading the index, you may discover mistakes, which
should be corrected by changing the appropriate \verb|\index|
commands in the document and regenerating the {\tt ind} file.  If
there are problems that cannot be corrected in this way, you can
edit the {\tt ind} file directly.  However, such editing is
to be avoided because it must be repeated every time you generate a
new version of the index.

If you would like to have ``general'' and ``author'' indexes
separately, please see \sref{sec3.1}. For more details on index
generation, see \cite{lamp87}.

\section{Multiple Indexes}\label{sec3.1}\index{index!multiple indexes}

To create a ``general'' and an ``author'' index, include the following lines:

\begin{verbatim}
...
\usepackage{ws-multind}
\makeindex{general}
\makeindex{authors}
...
\index{authors}{Fairbairns, R.} %\aindx{Fairbairns, R.}
...
\index{general}{FAQs}           %\gindx{FAQ}
...
\printindex{general}{GENERAL INDEX}
\printindex{authors}{AUTHOR INDEX}
\end{verbatim}

To complete the job, compile your file as follows:

\begin{enumerate}
\item latex ws-book975x65
\item latex ws-book975x65
\item bibtex ws-book975x65\qquad(for bibtex users)
\item makeindex general
\item makeindex authors
\item latex ws-book975x65
\item latex ws-book975x65
\end{enumerate}


==> check.tex <==
%% Usage: Latex check.tex
%%
%% Utility to test if all the files required for WSPC book 9.75x6.5 project
%% are available in your present LaTeX path.
%%
%% - ws-book975x65.cls
%% - ws-crop975x65.sty
%% - ws-book-har.sty
%% - ws-book-var.sty
%% - ws-book-har.bst
%% - ws-book-van.bst
%% - ws-multind.sty
%% - ws-book-thm.sty
%% - rotating.sty
%% - crop.sty
%% - hyperref.sty
%% - boxedminipage.sty
%% - makeidx.sty

\newif\onerror
\typeout{*}
\typeout{1. Searching for LaTeX2e ... }
\ifx\documentclass\undefined
 \typeout{*}
 \typeout{* Fatal error occurred:}
 \typeout{*}
 \typeout{* The WS Book class can only be used with LaTeX2e}
 \typeout{*}
 \typeout{* Stopping...}
 \expandafter\stop
\else
 \typeout{   ... ok}
\fi

\def\next#1/#2/#3\next{#1#2}
\typeout{ }
\typeout{2.  Searching for LaTeX2e version ... }
\ifnum\expandafter\next\fmtversion\next<199612 \relax
 \typeout{*}
 \typeout{* Fatal error occurred:}
 \typeout{*}
 \typeout{* Your LaTeX version is quite outdated, \fmtversion.}
 \typeout{* The WS Book class can only be used with a recent version}
 \typeout{* of LaTeX2e, please upgrade your installation!}
 \typeout{*}
 \expandafter\stop
\else
 \ifnum\expandafter\next\fmtversion\next<199806 \relax
   \typeout{* Warning: }
   \typeout{*}
   \typeout{* Your LaTeX version is outdated, \fmtversion.}
   \typeout{* We believe that it will probably work, but if you encounter}
   \typeout{* problems you will need upgrade your installation.}
   \typeout{*}
   \typein{* Type <return> to continue ...}
   \errortrue
 \else
   \typeout{   ... ok}
 \fi
\fi

\typeout{ }
\typeout{3. Searching for ws-book975x65.cls ... }
\IfFileExists{ws-book975x65.cls}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{* ... ws-book975x65.cls, file not found! }
     \typeout{*}
     \typeout{* Fatal error occurred:}
     \typeout{*}
     \typeout{* The ws-book975x65 class file which is part of the WS Books distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* Stopping...}
     \typeout{*}
     \stop
}

\typeout{ }

\typeout{4. Searching for ws-crop975x65.sty ... }
\IfFileExists{ws-crop975x65.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... ws-crop975x65.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The ws-crop975x65 file which is part of the WS Books distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* Without this package you will not be able to typeset }
     \typeout{* your book in 975x65 trim size.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{5. Searching for ws-book-har.sty ... }
\IfFileExists{ws-book-har.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... ws-book-har.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The ws-book-har file which is part of the WS Books distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* Without this package you will not be able to typeset }
     \typeout{* your references in WS author-date format.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{6. Searching for ws-book-van.sty ... }
\IfFileExists{ws-book-van.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... ws-book-van.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The ws-book-van file which is part of the WS Books distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* Without this package you will not be able to typeset }
     \typeout{* your references in WS numbered format.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{7. Searching for ws-book-har.bst ... }
\IfFileExists{ws-book-har.bst}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... ws-book-har.bst, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The BiBTeX style file, ws-book-har.bst which is part of the}
     \typeout{* WS Books distribution must be installed in a directory which}
     \typeout{* is searched by LaTeX.}
     \typeout{*}
     \typeout{* Without this package you will not be able to BiBTeX your references}
     \typeout{* in WS author-date format. If you are not a BiBTeX user you may}
     \typeout{* ignore this warning message.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{8. Searching for ws-book-van.bst ... }
\IfFileExists{ws-book-van.bst}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... ws-book-van.bst, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The BiBTeX style file, ws-book-van.bst which is part of the WS Books distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* Without this package you will not be able to BiBTeX your references}
     \typeout{* in WS numbered format. If you are not a BiBTeX user you may}
     \typeout{* ignore this warning message.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }

\typeout{9. Searching for ws-multind.sty ... }
\IfFileExists{ws-multind.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... ws-multind.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The ws-multind package which is part of the WS Books distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* You can use the ws-book975x65 class without this package but }
     \typeout{* you can not use multiple indexes.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{10. Searching for ws-book-thm.sty ... }
\IfFileExists{ws-book-thm.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... ws-book-thm.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The ws-book-thm package which is part of the WS Books distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* You need this package to typeset your theorems in WS format.}
     \typeout{* Alternate option is `amsmath` package.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }

\typeout{11. Searching for rotating.sty ... }
\IfFileExists{rotating.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... rotating.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The rotating package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to use}
     \typeout{* sidewaysfigure and sidewaystable environments.}
     \typeout{* Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "rotating".}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{12. Searching for crop.sty ... }
\IfFileExists{crop.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... crop.sty, file not found! }
     \typeout{*}
     \typeout{*}
     \typeout{* The crop package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* This package is required for printing the crop marks.}
     \typeout{* Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "crop".}
     \typeout{*}
     \typeout{* Stopping...}
     \typeout{*}
     \stop
}

\typeout{ }
\typeout{13. Searching for hyperref.sty ... }
\IfFileExists{hyperref.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... hyperref.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The hyperref package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to produce a hyper-linked pdf output.}
     \typeout{* Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "hyperref".}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{14. Searching for boxedminipage.sty ... }
\IfFileExists{boxedminipage.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... boxedminipage.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The boxedminipage package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to use the boxedtxt}
     \typeout{* environment. Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "boxedminipage".}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{15. Searching for makeidx.sty ... }
\IfFileExists{makeidx.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... makeidx.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The makeidx package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to generate index.}
     \typeout{* Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "makeidx".}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }

\typeout{* Finished Testing *}
\typeout{ }
\onerror
\typeout{* Some of the file(s) required by WS was not found.}
\typeout{* Please review the above comments carefully and update your system.}
\typeout{*}
\typeout{* WS files can be downloaded from:}
\typeout{* http://www.worldscientific.com/page/authors/book-stylefiles}
\typeout{*}
\typeout{* Other TeX packages can be downloaded from:}
\typeout{* http://www.ctan.org/search.html}
\typeout{*}
\typeout{* For technical support, please email Rajesh <rajesh@wspc.com.sg>}
\typeout{*}
\typeout{*****************************************************************}
\typein{* Type <return> to continue ...} \else
\typeout{*****************************************************************}
\typeout{*}
\typeout{* All the files and packages required by WS was found,}
\typeout{* you may now proceed LaTeXing your files.}
\typeout{*}
\typeout{* For technical support, please email Rajesh <rajesh@wspc.com.sg>}
\typeout{*}
\typeout{*****************************************************************}
\fi
\stop
\endinput

